Turning Federated Learning Systems Into Covert Channels

Federated learning (FL) goes beyond traditional, centralized machine learning by distributing model training among a large collection of edge clients. These clients cooperatively train a global, e.g., cloud-hosted, model without disclosing their local, private training data. The global model is then shared among all the participants which use it for local predictions. In this paper, we put forward a novel attacker model aiming at turning FL systems into covert channels to implement a stealth communication infrastructure. The main intuition is that, during federated training, a malicious sender can poison the global model by submitting purposely crafted examples. Although the effect of the model poisoning is negligible to other participants, and does not alter the overall model performance, it can be observed by a malicious receiver and used to transmit a single bit.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

In the previous section, we have shown the practical feasibility of FL covert channels.
Still, the actual exploitation of our technique requires further discussion, e.g., in terms of defenses that an FL system can implement to mitigate the attack.

\subsection{Detectability}
The first step for the defender is to detect the existence of a covert channel.
Below, we discuss two possible mechanisms that FL servers can implement to find out whether covert channels are running.
Although several techniques exist, here we focus on classification accuracy monitoring and model anomaly detection.
The reason is that these approaches are stepping stones to implement many backdoor detection mechanisms~\cite{kairouz2019advances}.
%\gcnote{da rivedere}

\paragraph{Classification accuracy monitoring}

FL server can monitor whether the accuracy of the global model decreases over time to guess if a Sender is poisoning the model by transmitting data.
% For this purpose, the FL server might hold a suitable dataset or, alternatively, it can randomly select a trusted client, and ask it to measure the accuracy of the global model by means of its own dataset.
For this purpose, the FL server can either measure the accuracy of the global model on a dedicated validation set that it holds or, alternatively, it can randomly select a trusted client and ask it to validate the global model using the client's dataset.
In our experiments, we implemented the second strategy, where the trusted client is randomly selected among the honest ones.
In particular, we compare the accuracy measured by the trusted client when Sender is not transmitting ($k = 0$) against that measured during transmissions with 1, 5 and 10 channels. 
The results for NN and CNN are shown in Figures~\ref{fig:accuracytime} and~\ref{fig:accuracytimecnn}, respectively.

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\columnwidth]{pics/accuracy_over_time.eps}
%    \caption{Model accuracy with different number of parallel cover channels $k \in \{1,5,10\}$ with $\tau$ = NN, $n_c = 10$, $p_c = 0.5$).}
%    \label{fig:accuracytime}
%\end{figure}

\begin{figure}[t]
    \begin{tikzpicture}
\begin{axis}[name=a1, ymin=0.97, ymax=1, xmin=0, xmax=600, xlabel={}, ylabel={Accuracy}, x label style={at={(axis description cs:0.5,-0.1)},anchor=center},
    y label style={at={(axis description cs:0.03,0.5)}, anchor=center},
    set layers=standard,
    xmajorgrids=true,
    ymajorgrids=true,
    y label style={at={(0.1cm,-0.7cm)}, anchor=center},
    ytick align=outside,
    ytick align=inside,
    xtick={},
    ytick={0.97,0.98,0.99,1},
    xtick pos=left,
    ytick pos=left,
    yticklabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    height=3cm,
    width=\columnwidth,
    legend style={at={(0.995,0.97)},anchor=north east},
    legend columns=-1,
    ybar=0pt, bar width=0.1, bar shift=0pt,
    xticklabels={,,},
    legend style={nodes={scale=0.8, transform shape}}
]
\addplot[line legend,draw=red,smooth,thick] table [col sep=comma] {data/accuracy0.csv}; 
\addlegendentry{$k=0$};
\addplot[line legend,draw=blue!50,smooth,thick] table [col sep=comma] {data/accuracy1.csv}; 
\addlegendentry{$k=1$};
\end{axis}

\begin{axis}[name=a2, ymin=0.97, ymax=1, xmin=0, xmax=600, xlabel={}, ylabel={}, x label style={at={(axis description cs:0.5,-0.1)},anchor=center},
    set layers=standard,
    xmajorgrids=true,
    ymajorgrids=true,
    ytick align=outside,
    ytick align=inside,
    xtick={},
    ytick={0.97,0.98,0.99},
    xtick pos=left,
    ytick pos=left,
    yticklabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    height=3cm,
    width=\columnwidth,
    legend style={at={(0.995,0.97)},anchor=north east},
    legend columns=-1,
    ybar=0pt, bar width=0.1, bar shift=0pt,
    xticklabels={,,},
    legend style={nodes={scale=0.8, transform shape}},
    at={(0,0)}, anchor=above north west]
    
\addplot[line legend,draw=red,smooth,thick] table [col sep=comma] {data/accuracy0.csv};
\addlegendentry{$k=0$};
\addplot[line legend,draw=blue!50,smooth,thick] table [col sep=comma] {data/accuracy5.csv}; 
\addlegendentry{$k=5$};
\end{axis}

\begin{axis}[name=a3, ymin=0.97, ymax=1, xmin=0, xmax=600, xlabel={Time (FL rounds)}, ylabel={}, x label style={at={(axis description cs:0.5,-0.2)},anchor=center},
    y label style={at={(axis description cs:0.03,0.5)}, anchor=center},
    set layers=standard,
    xmajorgrids=true,
    ymajorgrids=true,
    ytick align=outside,
    ytick align=inside,
    xtick={100,200,300,400,500},
    ytick={0.97,0.98,0.99},
    xtick pos=left,
    ytick pos=left,
    yticklabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    height=3cm,
    width=\columnwidth,
    legend style={at={(0.995,0.97)},anchor=north east},
    legend columns=-1,
    ybar=0pt, bar width=0.1, bar shift=0pt,
    legend style={nodes={scale=0.8, transform shape}},
    at={(0,-1.42cm)}, anchor=above north west]
    
\addplot[line legend,draw=red,smooth,thick] table [col sep=comma] {data/accuracy0.csv};
\addlegendentry{$k=0$};
\addplot[line legend,draw=blue!50,smooth,thick] table [col sep=comma] {data/accuracy10.csv}; 
\addlegendentry{$k=10$};
\end{axis}

\iffalse %%% BLOCK COMMENT START
\begin{axis}[name=a4, ymin=0.97, ymax=1, xmin=0, xmax=600, xlabel={}, ylabel={}, x label style={at={(axis description cs:0.5,-0.1)},anchor=center},
    y label style={at={(axis description cs:0.03,0.5)}, anchor=center},
    ytick align=outside,
    ytick align=inside,
    xtick={},
    ytick={0.97,0.98,0.99},
    xtick pos=left,
    ytick pos=left,
    yticklabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    height=3cm,
    width=\columnwidth,
    legend style={at={(0.995,0.97)},anchor=north east},
    legend columns=-1,
    ybar=0pt, bar width=0.1, bar shift=0pt,
    xticklabels={,,},
    legend style={nodes={scale=0.8, transform shape}},
    at={(0,-2.84cm)}, anchor=above north west]
    
\addplot[line legend,draw=red,smooth,thick] table [col sep=comma] {data/accuracy0.csv};
\addlegendentry{0};
\addplot[line legend,draw=blue!25,smooth,thick] table [col sep=comma] {data/accuracy4.csv}; 
\addlegendentry{4};
\end{axis}

\begin{axis}[name=a5, ymin=0.97, ymax=1, xmin=0, xmax=600, xlabel={}, ylabel={}, x label style={at={(axis description cs:0.5,-0.1)},anchor=center},
    y label style={at={(axis description cs:0.03,0.5)}, anchor=center},
    ytick align=outside,
    ytick align=inside,
    xtick={},
    ytick={0.97,0.98,0.99},
    xtick pos=left,
    ytick pos=left,
    yticklabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    height=3cm,
    width=\columnwidth,
    legend style={at={(0.995,0.97)},anchor=north east},
    legend columns=-1,
    ybar=0pt, bar width=0.1, bar shift=0pt,
    xticklabels={,,},
    legend style={nodes={scale=0.8, transform shape}},
    at={(0,-4.26cm)}, anchor=above north west]
    
\addplot[line legend,draw=red,smooth,thick] table [col sep=comma] {data/accuracy0.csv};
\addlegendentry{0};
\addplot[line legend,draw=blue!25,smooth,thick] table [col sep=comma] {data/accuracy5.csv}; 
\addlegendentry{5};
\end{axis}

\begin{axis}[name=a6, ymin=0.97, ymax=1, xmin=0, xmax=600, xlabel={}, ylabel={Accuracy}, x label style={at={(axis description cs:0.5,-0.1)},anchor=center},
    y label style={at={(0cm,0cm)}, anchor=center},
    ytick align=outside,
    ytick align=inside,
    xtick={},
    ytick={0.97,0.98,0.99},
    xtick pos=left,
    ytick pos=left,
    yticklabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    height=3cm,
    width=\columnwidth,
    legend style={at={(0.995,0.97)},anchor=north east},
    legend columns=-1,
    ybar=0pt, bar width=0.1, bar shift=0pt,
    xticklabels={,,},
    legend style={nodes={scale=0.8, transform shape}},
    at={(0,-5.68cm)}, anchor=above north west]
    
\addplot[line legend,draw=red,smooth,thick] table [col sep=comma] {data/accuracy0.csv};
\addlegendentry{0};
\addplot[line legend,draw=blue!25,smooth,thick] table [col sep=comma] {data/accuracy6.csv}; 
\addlegendentry{6};
\end{axis}

\begin{axis}[name=a7, ymin=0.97, ymax=1, xmin=0, xmax=600, xlabel={}, ylabel={}, x label style={at={(axis description cs:0.5,-0.1)},anchor=center},
    y label style={at={(axis description cs:0.03,0.5)}, anchor=center},
    ytick align=outside,
    ytick align=inside,
    xtick={},
    ytick={0.97,0.98,0.99},
    xtick pos=left,
    ytick pos=left,
    yticklabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    height=3cm,
    width=\columnwidth,
    legend style={at={(0.995,0.97)},anchor=north east},
    legend columns=-1,
    ybar=0pt, bar width=0.1, bar shift=0pt,
    xticklabels={,,},
    legend style={nodes={scale=0.8, transform shape}},
    at={(0,-7.10cm)}, anchor=above north west]
    
\addplot[line legend,draw=red,smooth,thick] table [col sep=comma] {data/accuracy0.csv};
\addlegendentry{0};
\addplot[line legend,draw=blue!25,smooth,thick] table [col sep=comma] {data/accuracy7.csv}; 
\addlegendentry{7};
\end{axis}

\begin{axis}[name=a8, ymin=0.97, ymax=1, xmin=0, xmax=600, xlabel={}, ylabel={}, x label style={at={(axis description cs:0.5,-0.1)},anchor=center},
    y label style={at={(axis description cs:0.03,0.5)}, anchor=center},
    ytick align=outside,
    ytick align=inside,
    xtick={},
    ytick={0.97,0.98,0.99},
    xtick pos=left,
    ytick pos=left,
    yticklabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    height=3cm,
    width=\columnwidth,
    legend style={at={(0.995,0.97)},anchor=north east},
    legend columns=-1,
    ybar=0pt, bar width=0.1, bar shift=0pt,
    xticklabels={,,},
    legend style={nodes={scale=0.8, transform shape}},
    at={(0,-8.52cm)}, anchor=above north west]
    
\addplot[line legend,draw=red,smooth,thick] table [col sep=comma] {data/accuracy0.csv};
\addlegendentry{0};
\addplot[line legend,draw=blue!25,smooth,thick] table [col sep=comma] {data/accuracy8.csv}; 
\addlegendentry{8};
\end{axis}

\begin{axis}[name=a9, ymin=0.97, ymax=1, xmin=0, xmax=600, xlabel={}, ylabel={}, x label style={at={(axis description cs:0.5,-0.1)},anchor=center},
    y label style={at={(axis description cs:0.03,0.5)}, anchor=center},
    ytick align=outside,
    ytick align=inside,
    xtick={},
    ytick={0.97,0.98,0.99},
    xtick pos=left,
    ytick pos=left,
    yticklabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    height=3cm,
    width=\columnwidth,
    legend style={at={(0.995,0.97)},anchor=north east},
    legend columns=-1,
    ybar=0pt, bar width=0.1, bar shift=0pt,
    xticklabels={,,},
    legend style={nodes={scale=0.8, transform shape}},
    at={(0,-9.94cm)}, anchor=above north west]
    
\addplot[line legend,draw=red,smooth,thick] table [col sep=comma] {data/accuracy0.csv};
\addlegendentry{0};
\addplot[line legend,draw=blue!25,smooth,thick] table [col sep=comma] {data/accuracy9.csv}; 
\addlegendentry{9};
\end{axis}

\begin{axis}[name=a10, ymin=0.97, ymax=1, xmin=0, xmax=600, xlabel={Time (FL rounds)}, ylabel={}, x label style={at={(axis description cs:0.5,-0.2)},anchor=center},
    y label style={at={(axis description cs:0.03,0.5)}, anchor=center},
    ytick align=outside,
    ytick align=inside,
    xtick={100,200,300,400,500},
    ytick={0.97,0.98,0.99},
    xtick pos=left,
    ytick pos=left,
    yticklabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    height=3cm,
    width=\columnwidth,
    legend style={at={(0.995,0.97)},anchor=north east},
    legend columns=-1,
    ybar=0pt, bar width=0.1, bar shift=0pt,
    legend style={nodes={scale=0.8, transform shape}},
    at={(0,-11.36cm)}, anchor=above north west]
    
\addplot[line legend,draw=red,smooth,thick] table [col sep=comma] {data/accuracy0.csv};
\addlegendentry{0};
\addplot[line legend,draw=blue!25,smooth,thick] table [col sep=comma] {data/accuracy10.csv}; 
\addlegendentry{10};
\end{axis}

\fi  %%% BLOCK COMMENT END

\end{tikzpicture}
    \caption{Classification accuracy for $k \in \{1,5,10\}$, $\tau$ = NN, $n_c = 10$, $p_c = 0.5$.}
    \label{fig:accuracytime}
\end{figure}

\begin{figure}[t]
    \begin{tikzpicture}
\begin{axis}[name=a1, ymin=0.97, ymax=1, xmin=0, xmax=600, xlabel={}, ylabel={Accuracy}, x label style={at={(axis description cs:0.5,-0.1)},anchor=center},
    y label style={at={(axis description cs:0.03,0.5)}, anchor=center},
    set layers=standard,
    xmajorgrids=true,
    ymajorgrids=true,
    y label style={at={(0.1cm,-0.7cm)}, anchor=center},
    ytick align=outside,
    ytick align=inside,
    xtick={},
    ytick={0.97,0.98,0.99,1},
    xtick pos=left,
    ytick pos=left,
    yticklabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    height=3cm,
    width=\columnwidth,
    legend style={at={(0.995,0.03)},anchor=south east},
    legend columns=-1,
    ybar=0pt, bar width=0.1, bar shift=0pt,
    xticklabels={,,},
    legend style={nodes={scale=0.8, transform shape}}
]
\addplot[line legend,draw=red,smooth,thick] table [col sep=comma] {data/accuracy0-cnn.csv}; 
\addlegendentry{$k=0$};
\addplot[line legend,draw=blue!50,smooth,thick] table [col sep=comma] {data/accuracy1-cnn.csv}; 
\addlegendentry{$k=1$};
\end{axis}

\begin{axis}[name=a2, ymin=0.97, ymax=1, xmin=0, xmax=600, xlabel={}, ylabel={}, x label style={at={(axis description cs:0.5,-0.1)},anchor=center},
    set layers=standard,
    xmajorgrids=true,
    ymajorgrids=true,
    ytick align=outside,
    ytick align=inside,
    xtick={},
    ytick={0.97,0.98,0.99},
    xtick pos=left,
    ytick pos=left,
    yticklabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    height=3cm,
    width=\columnwidth,
    legend style={at={(0.995,0.03)},anchor=south east},
    legend columns=-1,
    ybar=0pt, bar width=0.1, bar shift=0pt,
    xticklabels={,,},
    legend style={nodes={scale=0.8, transform shape}},
    at={(0,0)}, anchor=above north west]
    
\addplot[line legend,draw=red,smooth,thick] table [col sep=comma] {data/accuracy0-cnn.csv};
\addlegendentry{$k=0$};
\addplot[line legend,draw=blue!50,smooth,thick] table [col sep=comma] {data/accuracy5-cnn.csv}; 
\addlegendentry{$k=5$};
\end{axis}

\begin{axis}[name=a3, ymin=0.97, ymax=1, xmin=0, xmax=600, xlabel={Time (FL rounds)}, ylabel={}, x label style={at={(axis description cs:0.5,-0.2)},anchor=center},
    y label style={at={(axis description cs:0.03,0.5)}, anchor=center},
    set layers=standard,
    xmajorgrids=true,
    ymajorgrids=true,
    ytick align=outside,
    ytick align=inside,
    xtick={100,200,300,400,500},
    ytick={0.97,0.98,0.99},
    xtick pos=left,
    ytick pos=left,
    yticklabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    height=3cm,
    width=\columnwidth,
    legend style={at={(0.995,0.03)},anchor=south east},
    legend columns=-1,
    ybar=0pt, bar width=0.1, bar shift=0pt,
    legend style={nodes={scale=0.8, transform shape}},
    at={(0,-1.42cm)}, anchor=above north west]
    
\addplot[line legend,draw=red,smooth,thick] table [col sep=comma] {data/accuracy0-cnn.csv};
\addlegendentry{$k=0$};
\addplot[line legend,draw=blue!50,smooth,thick] table [col sep=comma] {data/accuracy10-cnn.csv}; 
\addlegendentry{$k=10$};
\end{axis}

\end{tikzpicture}
    \caption{Classification accuracy for $k \in \{1,5,10\}$, $\tau$ = CNN, $n_c = 10$, $p_c = 0.5$.}
    \label{fig:accuracytimecnn}
\end{figure}

As expected, since Sender joins a well trained FL system, the trusted client accuracy when $k=0$ is stable over time.
This behavior is peculiar of our implementation, where convergence of the network is ensured by the fact that the entire dataset is given in advance and, apart from edge examples, no new examples can emerge.
In most real FL systems, accuracy is not guaranteed to be stable.
The reason is that fresh training examples are dynamically generated by the clients, e.g., by sampling the physical environment through sensors.

For this reason, here we focus on average classification accuracy.
For NN, when $k=0$ the average accuracy is 0.983.
In the other cases, average accuracy is 0.982 ($k=1$), 0.982 ($k=5$) and 0.980 $(k=10)$.
For CNN, the average accuracy values are 0.992 ($k=0$), 0.992 ($k=1$), 0.989 ($k=5$) and 0.988 ($k=10$).

Since transmissions only minimally affect the overall accuracy of the classifier, FL server can hardly discover a covert channel through this kind of monitoring.
With larger neural networks that are trained with dynamically generated examples, this approach is likely to be ineffective. 

% NN: 0 -> AVG: 0.983, STD: 0
% 1 -> 0.982, 0.002
% 5 -> 0.982, 0.001
% 10 -> 0.980, 0.002

% CNN: 0 -> AVG: 0.992, STD 0.002
% 1 -> 0.992, 0.001
% 5 -> 0.989, 0.001
% 10 -> 0.988, 0.002


\paragraph{Model anomaly detection}
%\gcnote{i modelli del sender sono diversi dagli altri?}
In this case, FL server measures whether the model returned by a client is anomalous w.r.t. the others.
Although, several metrics can be considered to detect anomalies from a set of observations, a common approach is to measure the distance between the elements of the reference domain~\cite{Thudumu20anomaly}.
Here, we consider a distance-based approach.
When harvesting local models, FL server computes their distance from the current global model.
Using the L2-norm (aka Euclidean norm) as distance function, the anomaly score of a client's local model $m_c$ w.r.t. the global model $m$ is given by $d_c = \lVert m_c - m \rVert_2$.\footnote{More precisely, this amounts to computing the L2-norm of the difference between the vectors of parameters of $m_c$ and $m$.}
Finally, the client $c'$ such that $d_{c'} = \max_c d_c$ is tagged as the outlier.

%\gcnote{questa def mi confonde un attimo}

\begin{figure}[t]
\begin{tikzpicture}
\begin{axis}[ymin=0, xmin=1, xmax=200, xlabel={Time (FL rounds)}, ylabel={$\max_c d_c$}, x label style={at={(axis description cs:0.5,-0.1)},anchor=center},
    y label style={at={(axis description cs:0.04,0.5)}, anchor=center},
    set layers=standard,
    xmajorgrids=true,
    ymajorgrids=true,
    ytick align=outside,
    samples at={0,10,...,200},
    xtick pos=left,
    ytick pos=left,
    yticklabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    height=5cm,
    width=\columnwidth,
    legend style={at={(0.99,0.98)},anchor=north east},
    legend columns=-1,
    ybar=0pt, bar width=0.1, bar shift=0pt,
    legend style={nodes={scale=0.8, transform shape}}
]
\addplot[draw=blue!50, fill=blue!50, select coords between index={1}{200}] table [col sep=comma] {data/anomaly.csv}; 
\addlegendentry{FP};
\addplot[draw=red, fill=red, select coords between index={1}{200}] table [col sep=comma] {data/anomalysnd.csv};
\addlegendentry{TP};
\end{axis}
\end{tikzpicture}
\caption{Anomalous local models detected over 200 FL rounds ($\tau$ = NN, $k=1$, $n_c =10$, $p_c=0.5$, $f=6$).}
\label{fig:anomaly}
\end{figure}

\begin{figure}[t]
\begin{tikzpicture}
\begin{axis}[ymin=0, xmin=1, xmax=200, xlabel={Time (FL rounds)}, ylabel={$\max_c d_c$}, x label style={at={(axis description cs:0.5,-0.1)},anchor=center},
    y label style={at={(axis description cs:0.04,0.5)}, anchor=center},
    set layers=standard,
    xmajorgrids=true,
    ymajorgrids=true,
    ytick align=outside,
    samples at={0,10,...,200},
    xtick pos=left,
    ytick pos=left,
    yticklabel style={font=\footnotesize},
    xticklabel style={font=\footnotesize},
    height=5cm,
    width=\columnwidth,
    legend style={at={(0.99,0.98)},anchor=north east},
    legend columns=-1,
    ybar=0pt, bar width=0.1, bar shift=0pt,
    legend style={nodes={scale=0.8, transform shape}}
]
\addplot[draw=blue!50, fill=blue!50, select coords between index={1}{200}] table [col sep=comma] {data/anomaly-cnn.csv}; 
\addlegendentry{FP};
\addplot[draw=red, fill=red, select coords between index={1}{200}] table [col sep=comma] {data/anomalysnd-cnn.csv};
\addlegendentry{TP};
\end{axis}
\end{tikzpicture}
\caption{Anomalous local models detected over 200 FL rounds ($\tau$ = CNN, $k=1$, $n_c =10$, $p_c=0.5$, $f=6$).}
\label{fig:anomaly-cnn}
\end{figure}

We tested the precision of this anomaly detection approach on covert channels implemented on top of both NN and CNN.
Again, as for accuracy monitoring, we must consider that our experiments are executed on well trained networks, where honest clients never submit new examples. 
Figures~\ref{fig:anomaly} and~\ref{fig:anomaly-cnn} show the maximum $d_c$ detected by the server during 200 FL rounds (with $k=1$, $n_c=10$, $p_c=0.5$ and $f=6$).
Red bars correspond to true positives (TP), i.e., rounds where Sender's model was recognized as teh outlier.
Instead, blue bars denote false positives (FP), i.e., when another client was tagged as anomalous.
In the case of NN, the server detected Sender $24$ times (TP), which results in a precision of $24/200 = 12\%$.
For CNN, TP $= 36$ and, thus, precision is $34/200 = 17\%$.

FL servers might resort to anomaly detection mechanisms as the one discussed above.
In principle, this approach may be more effective than accuracy monitoring.
Nevertheless, to remain undetected, the attacker can apply some strategies to minimize $d_c$.
For instance, during calibration, Receiver can behave as an honest client, train a local model with some examples, and sample its own anomaly score $d_r$.
Then, Receiver passes $d_r$ as a parameter to Sender, which uses it as a threshold to limit the local training when transmitting.
This technique is similar to the poisoning data rate control presented in~\cite{Nguyen20poisoning}.

%\gcnote{ci vorrebbe una conclusione di qualche tipo}

\subsection{Countermeasures}
Below, we discuss some possible strategies that FL server can implement to prevent or degrade covert channels.

\paragraph{Model Jamming}
%\gcnote{si può perturbare il modello globale, ma si impatta sulle performance del sistema}
Jamming is a common strategy for degrading the communications over an unprotected channel.
For instance, in wireless communications jamming can amount to emitting random noise over a certain frequency to interfere with the transmissions.
In our context, jamming is performed by the FL server on the global model.
This is achieved by introducing a random perturbation to the parameters of the global model before distributing it to the clients.
Clearly, large perturbations may effectively degrade the covert channel quality.
However, jamming comes at the price of reducing the client-side classification accuracy.

\paragraph{Segmentation}
%\gcnote{si possono avere più modelli globali, ma l'attaccante può registrare più device}
Another possible countermeasure is to split the FL system into isolated FL clusters.
If clusters do not share their global models, a Sender and a Receiver federated to different clusters cannot communicate.
The flip side is that, under reasonable assumptions, clustered FL systems cannot achieve the same performance of standard ones, e.g., in terms of rate of convergence and accuracy.
Also, isolated clusters prevent the propagation of new, locally emerging features.
This may be partially solved by periodically allowing clusters to share their models.
However, in this way, the connection between Sender and Receiver may be established again.

\subsection{Exploitability}

There are several exploitation scenarios for our covert channel.
The first one is that of remote malware control.
Usually, attackers willing to harvest data from infected devices need to establish a communication channel with a command and control server.
To avoid being identified, malware often resort to anonymous connections, e.g., via onion routing.
However, onion traffic can be identified and filtered.
Instead, if the infected device is federated to some FL system, it is very likely that traffic toward the FL server is authorized.

Even more worrisome, our attacker model has the potential to fill the \emph{air gap}.
This is an actual risk since $(i)$ FL clients often train their local model with some sensor-generated examples (e.g., microphones and cameras for speech and face recognition), and $(ii)$ our attacker model does not require Sender to \emph{physically} reside on a client as far as it can poison training data with a proper function $\psi$.
For instance, an attacker controlling a speaker may poison nearby client examples via ultrasounds, as in~\cite{Guri18mosquito}.
The investigation of this and other exploitation strategies account as future work.

==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}

In this section, we present our experimental results.
%\gcnote{url da anonimizzare}
The implementation of our covert channel, called \emph{FedExp}, is available at~\url{https://anonymous.4open.science/r/3b6f1d83-f182-4fb4-abf5-3f5b9ba08169/}.\footnote{Anonymized for blind review.}
%\gtnote{Una volta anonimizzato, lo metterei come footnote. Dopodiché, andrebbe forse cambiato anche il nome del repo per richiamare l'idea del covert channel}
%The testing environment is available as a docker image at~\url{https://hub.docker.com/repository/docker/gabrielec/fedexp}.\gcnote{da anonimizzare}

\subsection{Experimental setting}
\label{sec:exp-setting}
All the tests described in this section were executed on Docker containers running on a dedicated Intel\textregistered{} Xeon\textregistered{} Gold 5218 2.30GHz CPU with 64 GB of memory.
The implementation is based on the popular ML framework PyTorch \cite{pytorch}.
In our testing environment, we implement an FL system for handwritten digits classification.

\paragraph{Dataset description} The MNIST dataset~\cite{minstdataset} is one of the most popular datasets used as benchmark for training and testing image classifiers. 
It contains a total of 70,000 greyscale images of handwritten, single digits.
Digit images are taken from American Census Bureau employees and American high school students.
Usually, 60,000 images are used for training and the remaining 10,000 for testing. 
Images are represented by $28\times28$ matrices of bytes, each byte representing a single pixel (where $0$ is for background color, i.e., white, and $255$ for foreground color, i.e., black).

\paragraph{FL system parameters}

Our FL system is configured according to three parameters, i.e., the number of honest FL clients ($n_c$), the client selection probability ($p_c$), and the neural network architecture ($\tau$).

At startup, both the training and the test portions of the full MNIST dataset are uniformly distributed at random among the $n_c$ honest clients.
At each round, the server sends the current global model to all the clients; then it randomly selects $\lfloor p_c \cdot n_c\rfloor$ clients.
Thus, selected clients use their portion of the MNIST dataset to train their own local models.
Such local models are then sent back to the server, which aggregates them into an updated global model using the standard federated averaging aggregation function FedAvg~\cite{mcmahan2017aistats}.
%Eventually, the new global model is distributed to all the clients.

%\paragraph{Neural Networks description}
%\fpnote{Da rivedere la descrizione delle reti. Valutare se inserire immagini delle reti e se approfindire}

The FL system we implemented supports two different types of neural network architectures.
The first one is a fully connected Neural Network (NN)~\cite{backprop}, which is composed by three layers with 200 neurons each. 
The second one is a Convolutional Neural Network (CNN)~\cite{cnn,cnn2} with two convolutional layers, each one of size 3x3, and one fully connected output layer.
After each convolutional layer we use a Max Pool 2D layer with kernel size 2x2.
Both networks use a ReLU activation function, and are trained by minimizing Cross Entropy (CE) loss function via Stochastic Gradient Descent (SGD)~\cite{goodfellow2016dl}.

\paragraph{Attacker parameters}

Receiver is added to the FL system after 200 training rounds.
The frame size $f$ can be manually configured. 
Otherwise, during the calibration phase, Receiver automatically sets $f$ to the number of rounds that it takes to be selected $T=4$ times by the server.
Another parameter is the number $k$ of parallel covert channels to be established.
Receiver generates $k$ edge examples, one for each channel, to be used during the communication.
Each edge example is generated by applying one of the following two linear transformation functions to the randomly selected MNIST examples $\boldsymbol{x_1}$ and $\boldsymbol{x_2}$.
\begin{itemize} 
    \item $\psi_v(\boldsymbol{x_1}, \boldsymbol{x_2}, \alpha)$ combines the upper $\alpha$ fragment of $\boldsymbol{x_1}$ with the lower $(1-\alpha)$ fragment of $\boldsymbol{x_2}$.
    \item $\psi_h(\boldsymbol{x_1}, \boldsymbol{x_2}, \alpha)$ combines the leftmost $\alpha$ fragment of $\boldsymbol{x_1}$ with the rightmost $(1-\alpha)$ fragment of $\boldsymbol{x_2}$.
\end{itemize}

Functions $\psi_v$ and $\psi_h$ resemble the example function $\psi_e$ of Section~\ref{SEC:IMPL}. 
Figure~\ref{fig:sample-vmix} shows two edge examples generated with Algorithm~\ref{alg:binary} when executing $\psi_v$ and $\psi_h$ on MNIST pairs (\#22242, \#7596) and (\#32481, \#18198), respectively.
In the first case, the two original examples are both classified as 4, and the resulting edge example is classified between 9 and 4.
In the second case, the two original images are classified as 2, and the edge example is classified between 2 and 4.

\begin{figure}[t]
    \centering
    \begin{tabular}{|c|c|c|}
    \toprule
    \includegraphics[width=0.28\columnwidth]{pics/7596.png} &
    \includegraphics[width=0.28\columnwidth]{pics/22242.png}   &
    \includegraphics[width=0.28\columnwidth]{pics/22242+7596.png} \\
    \midrule
    \includegraphics[width=0.28\columnwidth]{pics/32481g.png} &
    \includegraphics[width=0.28\columnwidth]{pics/18198r.png}   &
    \includegraphics[width=0.28\columnwidth]{pics/32481g+18198r.png} \\
    \bottomrule
    \end{tabular}
    \caption{Applications of $\psi_v$ to examples \#22242 and \#7596 (top) and $\psi_h$ to examples \#32481 and \#18198 (bottom).}
    \label{fig:sample-vmix}
\end{figure}

%%% Numero di edge samples
For the generation of edge examples, we randomly selected pairs of pictures from the MNIST dataset and we applied Algorithm~\ref{alg:binary} with both $\psi_h$ and $\psi_v$.
Over $6,000$ considered pairs, we obtained $101$ edge examples.
Thus, among all possible pairs of MNIST examples, approximately 1.7\% might be used to create edge examples.
This amounts to millions of possible channel implementations with $\psi_v$ and $\psi_h$ over the whole MNIST dataset. 

When Receiver completes the calibration phase, Sender is configured with the generated channel parameters.
Then, Sender joins the FL client network, which now consists of $n_c + 2$ clients, and starts the transmission.
Transmission parameters include $n_b$, i.e., the number of bits to be sent on each channel.
By default, Sender automatically generates random bit sequences.
Optionally, instead of random bits, one can specify a fixed bit pattern $w$.
Finally, when selected for training, Sender trains its local model in the same way, e.g., same number of training epochs, as all the other clients.
The only difference resides in the training examples.
That is, we assume Sender to have the same computational power of honest clients.

Table~\ref{tab:parameters} summarizes the experiment parameters for the FL system (top) and the attacker (bottom).


%
% TAB: Parameter
\begin{table}[t]
\centering
\caption{Parameters of FL system (top) and attacker (bottom).}
\label{tab:parameters}
\begin{tabular}{l l l l c}
\hline
\cellcolor{gray!25}\textbf{Par.} & \cellcolor{gray!25}\textbf{Description} & \cellcolor{gray!25}\textbf{Range} & \cellcolor{gray!25}\textbf{Example} & \cellcolor{gray!25}\textbf{Default} \\ \hline
$n_c$ & Number of honest clients & $\mathbb{N}$ & 10, 50 & 10 \\
$p_c$ & Client selection probability & $[0,1]$ & 0.1, 0.5  & 0.5 \\
$\tau$ & Neural network type & NN,CNN & NN & NN \\
%$n_e$ & Number of training epochs & $\mathbb{N}$ & 10, 20 & 10 \\
\hline
$f$ & Frame size & $\mathbb{N}$ & 6, 8 & auto \\
$k$ & Number of channels & $\mathbb{N}$ & 10, 20 & 1 \\
$n_b$ & Transmission length (bits) & $\mathbb{N}$ & 10, 100 & 10 \\
$w$ & Transmission pattern & $(0|1)^\ast$ & 10, 101 &  auto \\
\hline
\end{tabular}
\end{table}


\subsection{Results}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{pics/error-rate-probability-merged.eps}
    \caption{Single channel BER for NN (top), and for CNN (bottom).}
    \label{fig:errorate}
\end{figure}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{pics/error-rate-probability.eps}
%     \caption{Single channel BER for NN.}
%     \label{fig:errorate}
% \end{figure}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{pics/error-rate-probability_cnn.eps}
%     \caption{Single channel BER for CNN.}
%     \label{fig:erroratecnn}
% \end{figure}
%\fpnote{aggiungere dettaglio sul numero di esperimenti}
% aggiunto in footnote.
We start by assessing channel quality in terms of BER and SNR.
The box diagram\footnote{Each box represents 5 distinct experiments.} of Figures~\ref{fig:errorate} shows single channel BER measured on NN (top) and CNN (bottom) under different settings.
In particular, we consider $n_c \in \{10,50\}$, $p_c \in \{0.1, 0.2, 0.3, 0.4, 0.5\}$, $n_b = 100$ and $f$ automatically computed by Receiver.
%Each experiment is repeated 5 times.

Under the same settings described above, Figures~\ref{fig:avgber} and~\ref{fig:avgbercnn} show the average BER accumulated over 10-bits transmission slots.
%
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{pics/error-rate_over_time.pdf}
    \caption{Average BER on NN for 10-bits transmission slots.}
    \label{fig:avgber}
\end{figure}
%
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{pics/error-rate_over_time_cnn.pdf}
    \caption{Average BER on CNN for 10-bits transmission slots.}
    \label{fig:avgbercnn}
\end{figure}
%
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{pics/frame_length-probability-merged.eps}
    \caption{Receiver frame length estimation on NN (top) and CNN (bottom).}
    \label{fig:framesize}
\end{figure}
%
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{pics/frame_length-probability.eps}
%     \caption{Receiver frame length estimation on NN.}
%     \label{fig:framesize}
% \end{figure}
%
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{pics/frame_length-probability_cnn.eps}
%     \caption{Receiver frame length estimation on CNN.}
%     \label{fig:framesizecnn}
% \end{figure}
%
Results show that, when $p_c > 0.1$, BER tends to stay below 6\% already with the default heuristics for estimating $f$. 
%\st{is already sufficient to achieve adequate BER values.}\gcnote{aggiungerei la percentuale di esperimenti con BER minore di una soglia, es. 5\%}
Nevertheless, the attacker can achieve better performance by searching for optimal values of $f$ (as discussed in Section~\ref{SEC:IMPL}, BER is mainly affected by the choice of $f$).
Figures~\ref{fig:framesize} shows the frame size estimated at calibration time for the NN (top) and CNN (bottom) experiments presented above.
Instead, Figures~\ref{fig:berframenn} and~\ref{fig:berframecnn}, depict the cumulative BER for transmissions with increasing values of $f$, from 6 to 15.
Interestingly enough, NN and CNN exhibit different behaviors, which confirm our expectation that finding the optimal value of $f$ is non-trivial.
In particular, under the same settings, CNN tends to behave monotonically, i.e., increasing $f$ reduces BER, while NN does not exhibit e regular behavior.
The experiments suggest that the optimal frame size in the considered interval is $f = 7$ for NN and $f = 12$ for CNN.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{pics/error-rate-probability-frame_w_a.eps}
    \caption{BER using different frame sizes ($\tau =$ NN, $n_b = 100$, $n_c=10$, $p_c=0.5$).}
    \label{fig:berframenn}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{pics/error-rate-probability-frame_cnn.eps}
    \caption{BER using different frame sizes ($\tau =$ CNN, $n_b = 100$, $n_c=10$, $p_c=0.5$).}
    \label{fig:berframecnn}
\end{figure}

%\gcnote{la figura sui pattern forse non va messa qui}
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{pics/error-rate-patterns_both.eps}
    \caption{BER using different transmission patterns $w\in$ \{00, 0F, 55, FF, Random\} for both $\tau = $NN and $\tau =$ CNN  ($n_b = 100$, $n_c=10$, $p_c=0.5$, $f=7$ and $f=12$, for NN and CNN, respectively).}
    \label{fig:berpattern}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{pics/error-rate-patterns.eps}
%     \caption{BER using different byte patterns: 00, 0F, 55, FF and random ($\tau =$ NN, $n_b = 100$, $n_c=10$, $p_c=0.5$, $f=7$).}
%     \label{fig:berpattern}
% \end{figure}

Transmitted bit sequences may also impact on the communication quality.
An example of BER for different transmission patterns is shown in Figure~\ref{fig:berpattern}.
There, we considered five different patterns of transmitted bytes, i.e., 00, 0F, 55, FF and Random, for both NN and CNN.
In both cases, we set $f$ to the optimal values given above, i.e., $7$ and $12$ for NN and CNN, respectively.
As one might expect, 00 pattern results in the minimum BER.
The reason is that, since the FL system is well-trained, in most cases Sender does not need to poison the global model at all.
However, different patterns seem to slightly affect BER in NN, which still stays below 4\%, and to have almost no effect on CNN.
These results highlight that different types of network may change the behavior of the channel.
In general, finding the optimal channel parameter may require the attacker to carry out transmission tests such as the previous ones.
Nevertheless, this operation is allowed under our attacker model.
%\gcnote{commentare risultati}

The number of parallel covert channels that a FL system can support is another crucial aspect.
The reason is that the number of parallel covert channels represents the total transmission bandwidth.
Intuitively, we expect that an FL system can only host a finite number of channels before the model is saturated and the communication quality decays. 
%\ssnote{Non diciamo che aumentando il numero dei canali possiamo avere un aumento della capacità del canale?}
Figure~\ref{fig:bermulti} shows the increase of BER over the first 20 channels in NN, where the average BER increases with $k$. 
A similar behavior is represented in Figure~\ref{fig:bermulticnn} for CNN.  

%
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{pics/error-rate-probability-multi.eps}
    \caption{BER variation over the number of parallel covert channels $k$ (with $\tau$ = NN, $n_c = 10$, $p_c = 0.5$).}
    \label{fig:bermulti}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{pics/error-rate-probability-multi-cnn.eps}
    \caption{BER over the number of parallel covert channels $k$ (with $\tau$ = CNN, $n_c = 10$, $p_c = 0.5$).}
    \label{fig:bermulticnn}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{pics/snr_ber.eps}
    \caption{The SNR versus BER on NN and CNN.}
    \label{fig:snrber}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{pics/snr_cap.eps}
    \caption{The SNR versus channel capacity (C) for NN and CNN.}
    \label{fig:snrcap}
\end{figure}

%\gcnote{cambiare y label in fig. \ref{fig:snrcap}}
  
%\gcnote{spiegare brevemente come sono stati aggregati i dati}
Finally, we tested our definition of SNR (see Section~\ref{SEC:CHARAT}) as an indicator of the covert channel quality.
To this aim we compared SNR versus BER and capacity.
In both cases, for all the simulations, $(i)$ we computed the SNR, and $(ii)$ we binned SNR in $5$ dB intervals.
Then, for each bin, we computed the average BER (capacity, respectively).
Figure~\ref{fig:snrber} illustrates the BER when SNR increases, for both NN and CNN, under the settings presented above. 
Under the same settings, Figure~\ref{fig:snrcap} shows the relation between the SNR and channel capacity $C$.
Our experiments show that higher values of SNR result in better communications, both in terms of lower BER and higher successful transmission rate.
This trend follows the expected behavior of a channel in the classical information theory~\cite{Proakis2007digital}.
Thus, our experiments confirm that \eqref{EQ:SNR} is an appropriate definition of SNR.
%Moreover, according to the above results, covert channels built on NN perform slightly better than those running on CNN. 

% \simone{BER curves describe the performance of the communication through the covert channel.}
% \gcnote{questa parte va spiegata meglio, a partire dal perché: cosa vogliamo far vedere?}
% %We observe that BER comes down by increasing the SNR and also NN achieved a better perfomance.
% Also, Figure~\ref{fig:snrcap} depicts the relation between the SNR and channel capacity $C$.
% Increasing the intensity of the differential signal $z$ results in augmenting the channel capacity (in bits per \simone{frame}). 
% The reason is that larger amplitude of $z$ makes the transmission less influenced by channel noise.
% \simone{It is interesting to note that the general behaviour of the $C$ as function of SNR of this covert channel it is the same as what we would have for
% a traditional digital communication.}
% \gcnote{non è chiarissimo e soprattutto non si capisce bene perché è interessante}
% \fpnote{io metterei che il comportamento del canale rispetto a SNR e capacity rispetta il comportamento di un canale di comunicazioni implementati su mezzi standard di comunicazione. Confermando la bontà della nostra implementazione.}

Our experiments highlight that covert channels can be instantiated on both NN and CNN networks, although NN provides better performances in terms of channel quality, transmission rate ($f$) and bandwidth.
However, further investigation is necessary to find parameters, e.g., frame size and edge examples, that maximize the performance of a channel.
Since some optimizations can be implemented, we believe that the channel quality can be further improved.

